BiSON data preparation: A correction for differential extinction and the weighted averaging of contemporaneous data

The Birmingham Solar Oscillations Network (BiSON) has provided high-quality high-cadence observations from as far back in time as 1978. These data must be calibrated from the raw observations into radial velocity and the quality of the calibration has a large impact on the signal-to-noise ratio of the final time series. The aim of this work is to maximise the potential science that can be performed with the BiSON data set by optimising the calibration procedure. To achieve better levels of signal-to-noise ratio we perform two key steps in the calibration process: we attempt a correction for terrestrial atmospheric differential extinction; and the resulting improvement in the calibration allows us to perform weighted averaging of contemporaneous data from different BiSON stations. The improvements listed produce significant improvement in the signal-to-noise ratio of the BiSON frequency-power spectrum across all frequency ranges. The reduction of noise in the power spectrum will allow future work to provide greater constraint on changes in the oscillation spectrum with solar activity. In addition, the analysis of the low-frequency region suggests we have achieved a noise level that may allow us to improve estimates of the upper limit of g-mode amplitudes.

==> tmp <==
Query Results from the ADS Database


Retrieved 1 abstracts, starting with number 1.  Total number selected: 1.

@ARTICLE{2010A&ARv..18..197A,
   author = {{Appourchaux}, T. and {Belkacem}, K. and {Broomhall}, A.-M. and 
	{Chaplin}, W.~J. and {Gough}, D.~O. and {Houdek}, G. and {Provost}, J. and 
	{Baudin}, F. and {Boumier}, P. and {Elsworth}, Y. and {Garc{\'{\i}}a}, R.~A. and 
	{Andersen}, B.~N. and {Finsterle}, W. and {Fr{\"o}hlich}, C. and 
	{Gabriel}, A. and {Grec}, G. and {Jim{\'e}nez}, A. and {Kosovichev}, A. and 
	{Sekii}, T. and {Toutain}, T. and {Turck-Chi{\`e}ze}, S.},
    title = "{The quest for the solar g modes}",
  journal = {\aapr},
archivePrefix = "arXiv",
   eprint = {0910.0848},
 primaryClass = "astro-ph.SR",
 keywords = {Sun, Theory, Data analysis, g modes},
     year = 2010,
    month = feb,
   volume = 18,
    pages = {197-277},
      doi = {10.1007/s00159-009-0027-z},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26ARv..18..197A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


